Group $K$-Means

We study how to learn multiple dictionaries from a dataset, and approximate any data point by the sum of the codewords each chosen from the corresponding dictionary. Although theoretically low approximation errors can be achieved by the global solution, an effective solution has not been well studied in practice. To solve the problem, we propose a simple yet effective algorithm \textit{Group $K$-Means}. Specifically, we take each dictionary, or any two selected dictionaries, as a group of $K$-means cluster centers, and then deal with the approximation issue by minimizing the approximation errors. Besides, we propose a hierarchical initialization for such a non-convex problem. Experimental results well validate the effectiveness of the approach.

==> two_criteria.tex <==

Two criteria are used to evaluate the approaches: relative distortion 
and recall for approximate nearest search. 
The relative distortion 
is defined as the objective function of Eqn.~\ref{eqn:gkmeans_obj} with the solved optimal solutions divided 
by $\sum_{\mathbf{x} \in \mathcal{X}} \|\mathbf{x}\|_2^2$.
This indicator is important to data compression, and the performance is better with a lower distortion.
For the second criterion, we follow~\cite{WangWSXSL14} and estimate the distance between a query $\mathbf{q}$ 
and a database point $\mathbf{x}$ with the code $\{k_c\}$ as
\begin{align}
\|\mathbf{q} - \sum_{c}\mathbf{d}_{k_c}^{c}\|_2^2 \approx \frac{1}{2} \|\mathbf{q}\|_2^2 - \sum_{c}\mathbf{q}^{T} \mathbf{d}_{k_c}^{c}
+ \frac{1}{2}\sum_{c_1, c_2}{\mathbf{d}_{k_{c_1}}^{c_1}}^{T} \mathbf{d}_{k_{c_2}}^{c_2}.
\end{align}
The first term is constant to all the database points and can be ignored, while the last term
can be pre-computed once for all the queries. The second term can be obtained by pre-computing a lookup table
which contains $\{\mathbf{q}^{T} \mathbf{d}_{k}^{c} \}_{k = 1, c = 1}^{K, C}$. Then, the approximate distance
is obtained by table lookups and additions. All the database points are ranked based on the
approximate distance and the recall is 
the proportion over all the queries where the true nearest neighbor (based on 
Euclidean distance)
falls within the top ranked points. 


%The superior of the gk-means(2, h) is shown in Fig.~\ref{fig:recall} w.r.t. the recall
%for approximate nearest neighbor (ANN) search.
